MedReadMe: A Systematic Study for Fine-grained Sentence Readability in Medical Domain

Medical texts are notoriously challenging to read. Properly measuring their readability is the first step towards making them more accessible. In this paper, we present a systematic study on fine-grained readability measurements in the medical domain at both sentence-level and span-level. We introduce a new dataset MedReadMe, which consists of manually annotated readability ratings and fine-grained complex span annotation for 4,520 sentences, featuring two novel "Google-Easy" and "Google-Hard" categories. It supports our quantitative analysis, which covers 650 linguistic features and automatic complex word and jargon identification. Enabled by our high-quality annotation, we benchmark and improve several state-of-the-art sentence-level readability metrics for the medical domain specifically, which include unsupervised, supervised, and prompting-based methods using recently developed large language models (LLMs). Informed by our fine-grained complex span annotation, we find that adding a single feature, capturing the number of jargon spans, into existing readability formulas can significantly improve their correlation with human judgments. The data is available at tinyurl.com/medreadme-repo

==> backup_section1_comments.tex <==

Medical texts are notoriously challenging to read. Properly measuring their readability is the first step toward making them more accessible. Here, we present the first systematic study on fine-grained readability measurements on both sentence and span levels in the medical domain, including an annotated dataset, investigation of existing corpus, metrics, and trained models. We first introduce \medcsi, which consists of manually annotated readability ratings for 1,924 sentences, and fine-grained complex span annotation on 4,520 sentences, featuring two novel ``Google-Easy'' and ``Google-Hard'' categories.  Our analysis reveals the significant variations in readability and jargon distribution across the 15 widely-used medical text simplification resources.
Enabled by our high-quality annotated dataset, we evaluate state-of-the-art readability metrics, including unsupervised, supervised, and prompting-based methods using recently developed large language models (LLMs). To further improve their performance, we find that adding a single feature, capturing the ``number of jargon'', into existing readability formulas significantly improves their correlation with human judgments and stability.   We will make our dataset and code publicly available. 





\noindent Comprehending medical documents can be a challenging task due to their technical nature and the extensive use of specialized terminology \cite{zeng2005text}. \wx{I like this first sentence at the beginning.}
Patients who cannot understand medical articles or doctor's notes \wx{We are not doing doctor's notes in our paper, this may open the door of attacks from the reviewers. There is one point we want to argue, why lay people would benefit from reading professional medical documents (majority of data used in this paper) and/or Wikipedia articles. Check \href{https://kyleclo.github.io/assets/pdf/paper-plain-making-medical-research-papers-approachable-to-healthcare-consumers-with-natural-language-processing.pdf}{this} and \href{https://arxiv.org/pdf/2305.12532.pdf}{this paper} for inspiration.} will face increased anxiety \cite{graham2008patients} and lower healthcare outcomes \cite{ links2019surgeon}. \wx{I like the transition here using ``as the first step''.} As the first step to making them more accessible, properly measuring the readability of medical texts is crucial \cite{rooney2021readability,echuri2022readability}. However, widely-used evaluation metrics such as FKGL, ARI, and SMOG \cite{kincaid1975derivation, smith1967automated, mc1969smog}, assuming longer words and sentences are harder to understand \wx{I think this argument on length is a bit hard to defend, as any methods include yours would need length}, have been shown to work poorly \wx{thought they work okay, though not great} in the medical domain \cite{wilson2009readability, jindal2017assessing,devaraj2021paragraph}. \wx{what we need to convey is that ... people do not yet have a good data resource for measuring/evaluating medical text's readability methods, or by studying finer-grained span-level information we can improve. } Recent studies \cite{arase-etal-2022-cefr, naous2023towards} also indicate that sentences of similar lengths can have very different readability ratings, especially for professional domains, such as medicine. \wx{we may need to nail down a different research question here -- I first thought human factors (who is rating it) will be the biggest factor} A persistent research question arises:  \textit{beyond length, what other factors affect the readability ratings of medical texts?}






\wx{I kind of like this framing, yet, we may need to carefully tweak a bit of the wording (writing more defensively), as readers may not believe there is no prior'' study for sentence readability in the medical domain''} Here, we present the first systematic study for sentence readability in the medical domain, including annotated data, analysis, improvements to existing metrics, and trained models. As demonstrated in Figure 1, we first construct \medcsi, consisting of 1,924 readability ratings at sentence-level, in addition to fine-grained complex span annotation on 4,520 sentences (\S \ref{section:dataset-construction}). It covers 15 resources that have been widely used in medical text simplification research, including scientific papers, systematic reviews, and medical references. The readability ratings are annotated using a rank-and-rate interface \cite{maddela-etal-2023-lens} based on the CEFR scale \cite{arase-etal-2022-cefr}, which is shown to be more reliable than the other methods \cite{naous2023towards}. 
To capture the reasons behind the sentence-level rating, we ask annotators to highlight any span that they find is hard to understand, and categorize the reason using a 7-class taxonomy that we developed. Considering that ``the majority of U.S. adults search for health information online and nearly eight-in-ten (77\%) of them began at a search engine'',\footnote{\url{https://tinyurl.com/seek-health-info-online}}
 we introduce two ``Google-Easy'' and ``Google-Hard'' classes, providing a fresh perspective beyond binary or 5-point Likert scales.



\begin{figure*}[pht!]
    \centering
    \includegraphics[width=\linewidth]{figs/21.pdf}
    \vspace{-18pt}
    \caption{The distribution of average sentence readability \textcolor{myblue}{(boxplot on the left y-axis)} and the average number of jargon spans per category \textcolor{mygreen}{(stacked barplot on the right y-axis)} in each sentence across both complex and simple versions for 15 commonly used text simplification resources. The readability of each resource varies significantly. The simplified texts from some venues are harder to read than the complex versions of some other sources }
    \label{fig:readability-jargon-distribution}
    \vspace{-14pt}
\end{figure*}


Our work addresses three limitations in prior work. (1) Previous research assumes all sentences in one document have the same readability, which is shown to be flawed \cite{arase-etal-2022-cefr, cripwell2023simplicity}; (2) Recent work with sentence-level ratings mainly covers data from one or two general domains, such as Wikipedia \cite{de-clercq-hoste-2016-mixed}, news \cite{vstajner2017automatic, brunato-etal-2018-sentence}, and textbooks for EFL learners \cite{arase-etal-2022-cefr}, which are very different from specialized fields, such as medicine \cite{choi2007multidisciplinarity}; (3) Existing work separated the research on sentence readability and complex jargon terms, therefore failing to study the possible correlations between them \cite{kwon-etal-2022-medjex, naous2023towards}.  

Enabled on our high-quality corpus, we first scrutinize 15 popular medical simplification resources. We discover that not all complex texts are equally ``simplified'', as the plain texts from some corpora are more challenging to read than the complex texts from other resources. Furthermore, the topics of some resources may not be directly relevant to laypersons (\S \ref{section:variance-of-readability}). Hence, we argue that the current practice of simply combining all available data for training should be re-considered, and the decision to include a corpus should be made with caution after considering the intended audiences’ desired simplification level and the application domain.  




For existing metrics, we find that unsupervised methods based on lexical features perform poorly, whereas RSRS score \cite{martinc2021supervised} based on a weighted sum of words' log probability achieves better performance. Prompting large language models such as GPT4  and Llama2 \cite{touvron2023llama} with 5-shot shows strong performance, yet outperformed by fine-tuned models in a much smaller size (\S \ref{section:evaluating-existing-readability}). Our analysis reveals that medical jargon significantly impacts readability, even more so than the average sentence or word length (\S \ref{section:jargon-drive-up}). 
To incorporate this intuition, we add a single feature that captures the  ``number of jargon'' in a sentence into existing readability formulas, and find it significantly improves their correlations with human judgments as well as stability. With predictions from our best complex span identification model (\S \ref{sec:cwi_experiment}), the proposed method achieved a 0.847 (+15\%) Pearson correlation for supervised metrics and 0.759 (+12\%) for the unsupervised ones (\S \ref{section:add-jar-method}).





